Demystifying and Assessing Code Understandability in Java Decompilation

Decompilation, the process of converting machine-level code into readable source code, plays a critical role in reverse engineering. Given that the main purpose of decompilation is to facilitate code comprehension in scenarios where the source code is unavailable, the understandability of decompiled code is of great importance. In this paper, we propose the first empirical study on the understandability of Java decompiled code and obtained the following findings: (1) Understandability of Java decompilation is considered as important as its correctness, and decompilation understandability issues are even more commonly encountered than decompilation failures. (2) A notable percentage of code snippets decompiled by Java decompilers exhibit significantly lower or higher levels of understandability in comparison to their original source code. (3) Unfortunately, Cognitive Complexity demonstrates relatively acceptable precision while low recall in recognizing these code snippets exhibiting diverse understandability during decompilation. (4) Even worse, perplexity demonstrates lower levels of precision and recall in recognizing such code snippets. Inspired by the four findings, we further proposed six code patterns and the first metric for the assessment of decompiled code understandability. This metric was extended from Cognitive Complexity, with six more rules harvested from an exhaustive manual analysis into 1287 pairs of source code snippets and corresponding decompiled code. This metric was also validated using the original and updated dataset, yielding an impressive macro F1-score of 0.88 on the original dataset, and 0.86 on the test set.

==> listings/Bukkit-MemorySection-cfr.tex <==
\begin{lstlisting}[style=Java, float, floatplacement=H, caption={The decompilation result of \autoref{lst:Bukkit-MemorySection-original-bytecode} with CFR.}, label={lst:Bukkit-MemorySection-cfr},belowskip=0\baselineskip] 
@Override
public Set<String> getKeys(boolean deep) {
    ConfigurationSection defaults;
    LinkedHashSet<String> result = new LinkedHashSet<String>();
    Configuration root = this.getRoot();
    if (root != null && root.options().copyDefaults() && (defaults = this.getDefaultSection()) != null) {
        result.addAll(defaults.getKeys(deep));
    }
    this.mapChildrenKeys(result, this, deep);
    return result;
}
\end{lstlisting}

==> listings/Bukkit-MemorySection-fernflower.tex <==
\begin{lstlisting}[style=Java, float, floatplacement=H, caption={The decompilation result of \autoref{lst:Bukkit-MemorySection-original-bytecode} with Fernflower.}, label={lst:Bukkit-MemorySection-fernflower},belowskip=0\baselineskip] 
public Set<String> getKeys(boolean deep) {
  Set<String> result = new LinkedHashSet();
  Configuration root = this.getRoot();
  if (root != null && root.options().copyDefaults()) {
     ConfigurationSection defaults = this.getDefaultSection();
     if (defaults != null) {
        result.addAll(defaults.getKeys(deep));
     }
  }
  this.mapChildrenKeys(result, this, deep);
  return result;
}
\end{lstlisting}

==> listings/Bukkit-MemorySection-jadx.tex <==
\begin{lstlisting}[style=Java, float, floatplacement=H, caption={The decompilation result of \autoref{lst:Bukkit-MemorySection-original-bytecode} with Jadx.}, label={lst:Bukkit-MemorySection-jadx},belowskip=0\baselineskip] 
@Override // org.bukkit.configuration.ConfigurationSection
public Set<String> getKeys(boolean deep) {
    ConfigurationSection defaults;
    Set<String> result = new LinkedHashSet<>();
    Configuration root = getRoot();
    if (root != null && root.options().copyDefaults() && (defaults = getDefaultSection()) != null) {
        result.addAll(defaults.getKeys(deep));
    }
    mapChildrenKeys(result, this, deep);
    return result;
}
\end{lstlisting}

==> listings/Bukkit-MemorySection-original-bytecode.tex <==
\begin{lstlisting}[style=Java, float, floatplacement=H, caption={Excerpt of disassembled bytecode from code in \autoref{lst:Bukkit-MemorySection-original}.}, label={lst:Bukkit-MemorySection-original-bytecode},belowskip=0\baselineskip] 
public java.util.Set<java.lang.String> getKeys(boolean);
     0: new           #76                 // class java/util/LinkedHashSet
     3: dup
     4: invokespecial #78                 // Method java/util/LinkedHashSet."<init>":()V
     7: astore_2
     8: aload_0
     9: invokevirtual #79                 // Method getRoot: ()Lorg/bukkit/configuration/Configuration;
    12: astore_3
    13: aload_3
    14: ifnull        55
    17: aload_3
    18: invokeinterface #80,  1           // InterfaceMethod org/bukkit/configuration/Configuration.options: ()Lorg/bukkit/configuration/ConfigurationOptions;
    23: invokevirtual #84                 // Method org/bukkit/configuration/ConfigurationOptions.copyDefaults:()Z
    26: ifeq          55
    29: aload_0
    30: invokevirtual #90                 // Method getDefaultSection: ()Lorg/bukkit/configuration/ConfigurationSection;
    33: astore        4
    35: aload         4
    37: ifnull        55
    40: aload_2
    41: aload         4
    43: iload_1
    44: invokeinterface #94,  2           // InterfaceMethod org/bukkit/configuration/ConfigurationSection. getKeys:(Z)Ljava/util/Set;
    49: invokeinterface #96,  2           // InterfaceMethod java/util/Set.addAll:(Ljava/util/Collection;)Z
    54: pop
    55: aload_0
    56: aload_2
    57: aload_0
    58: iload_1
    59: invokevirtual #102                // Method mapChildrenKeys: (Ljava/util/Set; Lorg/bukkit/configuration/ConfigurationSection;Z)V
    62: aload_2
    63: areturn
\end{lstlisting}


==> listings/Bukkit-MemorySection-original.tex <==
\begin{lstlisting}[style=Java, float, floatplacement=H, caption={One method of Java class \texttt{org.bukkit.configuration.MemorySection}.}, label={lst:Bukkit-MemorySection-original},belowskip=0\baselineskip] 
public Set<String> getKeys(boolean deep) {
    Set<String> result = new LinkedHashSet<String>();
    Configuration root = getRoot();
    if (root != null && root.options().copyDefaults()) {
        ConfigurationSection defaults = getDefaultSection();
        if (defaults != null) {
            result.addAll(defaults.getKeys(deep));
        }
    }
    mapChildrenKeys(result, this, deep);
    return result;
}
\end{lstlisting}

==> listings/codec_CharSeq_cfr.tex <==
\textbf{}\begin{lstlisting}[style=Java, float, floatplacement=H, caption={Excerpt of \texttt{org.\allowbreak{}apache.\allowbreak{}commons.\allowbreak{}codec.\allowbreak{}binary.\allowbreak{}CharSequenceUtils} produced by CFR}, label={lst:charseq-cfr},belowskip=-6\baselineskip,escapeinside=``]
public class CharSequenceUtils {
    static boolean regionMatches(...) {
        if (...) {
            [...]
        }
        [...]
        while (tmpLen-- > 0) {
            char c2;
            char c1;
            @@if ((c1 = cs.charAt(index1++)) == (c2 = substring.charAt(index2++))) continue;@@
            if (!ignoreCase) {
                return false;
            }
            @@if (Character.toUpperCase(c1) == Character.toUpperCase(c2) || Character.toLowerCase(c1) == Character.toLowerCase(c2)) continue;@@
            return false;
        }
        return true;
    }
}
\end{lstlisting}

==> listings/codec_CharSeq_cfr_ori.tex <==
\textbf{}\begin{lstlisting}[style=Java, float, floatplacement=H, caption={Excerpt of \texttt{org.\allowbreak{}apache.\allowbreak{}commons.\allowbreak{}codec.\allowbreak{}binary.\allowbreak{}CharSequenceUtils} produced by CFR}, label={lst:charseq-cfr},belowskip=-6\baselineskip,escapeinside=``]
public class CharSequenceUtils {
    static boolean regionMatches(CharSequence cs, boolean ignoreCase, int thisStart, CharSequence substring, int start, int length) {
        if (...) {
            [...]
        }
        int index1 = thisStart;
        int index2 = start;
        int tmpLen = length;
        while (tmpLen-- > 0) {
            char c2;
            char c1;
            @@if ((c1 = cs.charAt(index1++)) == (c2 = substring.charAt(index2++))) continue;@@
            if (!ignoreCase) {
                return false;
            }
            @@if (Character.toUpperCase(c1) == Character.toUpperCase(c2) || Character.toLowerCase(c1) == Character.toLowerCase(c2)) continue;@@
            return false;
        }
        return true;
    }
}
\end{lstlisting}

==> listings/codec_CharSeq_fernflower.tex <==
\textbf{}\begin{lstlisting}[style=Java, float, floatplacement=H, caption={Excerpt of \texttt{org.\allowbreak{}apache.\allowbreak{}commons.\allowbreak{}codec.\allowbreak{}binary.\allowbreak{}CharSequenceUtils} produced by Fernflower}, label={lst:charseq-fern},belowskip=-6\baselineskip,escapeinside=``]
public class CharSequenceUtils {
    static boolean regionMatches(...) {
        if (...) {
            [...]
        } @@else {@@
         [...]
         while(tmpLen-- > 0) {
            char c1 = cs.charAt(index1++);
            char c2 = substring.charAt(index2++);
            if (c1 != c2) {
               if (!ignoreCase) {
                  return false;
               }
               @@if (Character.toUpperCase(c1) != Character.toUpperCase(c2) && Character.toLowerCase(c1) != Character.toLowerCase(c2)) {@@
                  return false;
               }
            }
         }
         return true;
      @@}@@
    }
}
\end{lstlisting}

==> listings/codec_CharSeq_fernflower_ori.tex <==
\textbf{}\begin{lstlisting}[style=Java, float, floatplacement=H, caption={Excerpt of \texttt{org.\allowbreak{}apache.\allowbreak{}commons.\allowbreak{}codec.\allowbreak{}binary.\allowbreak{}CharSequenceUtils} produced by Fernflower}, label={lst:charseq-fern},belowskip=-6\baselineskip,escapeinside=``]
public class CharSequenceUtils {
    static boolean regionMatches(CharSequence cs, boolean ignoreCase, int thisStart, CharSequence substring, int start, int length) {
        if (...) {
            [...]
        } @@else {@@
         int index1 = thisStart;
         int index2 = start;
         int tmpLen = length;

         while(tmpLen-- > 0) {
            char c1 = cs.charAt(index1++);
            char c2 = substring.charAt(index2++);
            if (c1 != c2) {
               if (!ignoreCase) {
                  return false;
               }

               @@if (Character.toUpperCase(c1) != Character.toUpperCase(c2) && Character.toLowerCase(c1) != Character.toLowerCase(c2)) {@@
                  return false;
               }
            }
         }

         return true;
      @@}@@
    }
}
\end{lstlisting}

==> listings/codec_CharSeq_jadx.tex <==
\textbf{}\begin{lstlisting}[style=Java, float, floatplacement=H, caption={Excerpt of \texttt{org.\allowbreak{}apache.\allowbreak{}commons.\allowbreak{}codec.\allowbreak{}binary.\allowbreak{}CharSequenceUtils} produced by Jadx}, label={lst:charseq-jadx},belowskip=-6\baselineskip,escapeinside=``]
public class CharSequenceUtils {
    static boolean regionMatches(...) {
        if (...) {
            [...]
        }
        [...]
        @@while (true) {@@
            int i = tmpLen;
            tmpLen--;
            if (i > 0) {
                int i2 = index1;
                index1++;
                char c1 = cs.charAt(i2);
                int i3 = index2;
                index2++;
                char c2 = substring.charAt(i3);
                if (c1 != c2) {
                    if (!ignoreCase) {
                        return false;
                    }
                    @@if (Character.toUpperCase(c1) != Character.toUpperCase(c2) && Character.toLowerCase(c1) != Character.toLowerCase(c2)) {@@
                        return false;
                    }
                }
            } else {
                return true;
            }
        @@}@@
    }
}
\end{lstlisting}

==> listings/codec_CharSeq_jadx_ori.tex <==
\textbf{}\begin{lstlisting}[style=Java, float, floatplacement=H, caption={Excerpt of \texttt{org.\allowbreak{}apache.\allowbreak{}commons.\allowbreak{}codec.\allowbreak{}binary.\allowbreak{}CharSequenceUtils} produced by Jadx}, label={lst:charseq-jadx},belowskip=-6\baselineskip,escapeinside=``]
public class CharSequenceUtils {
    static boolean regionMatches(CharSequence cs, boolean ignoreCase, int thisStart, CharSequence substring, int start, int length) {
        if (...) {
            [...]
        }
        int index1 = thisStart;
        int index2 = start;
        int tmpLen = length;
        @@while (true) {@@
            int i = tmpLen;
            tmpLen--;
            if (i > 0) {
                int i2 = index1;
                index1++;
                char c1 = cs.charAt(i2);
                int i3 = index2;
                index2++;
                char c2 = substring.charAt(i3);
                if (c1 != c2) {
                    if (!ignoreCase) {
                        return false;
                    }
                    @@if (Character.toUpperCase(c1) != Character.toUpperCase(c2) && Character.toLowerCase(c1) != Character.toLowerCase(c2)) {@@
                        return false;
                    }
                }
            } else {
                return true;
            }
        @@}@@
    }
}
\end{lstlisting}

==> listings/codec_CharSeq_ori.tex <==
\textbf{}\begin{lstlisting}[style=Java, float, floatplacement=H, caption={Excerpt of \texttt{org.\allowbreak{}apache.\allowbreak{}commons.\allowbreak{}codec.\allowbreak{}binary.\allowbreak{}CharSequenceUtils}}, label={lst:charseq-ori}, escapechar=\¤,belowskip=-6\baselineskip]
public class CharSequenceUtils {
    static boolean regionMatches(...) {
        if (...) {
            [...]
        }
        [...]
        while (tmpLen-- > 0) {
            char c1 = cs.charAt(index1++);
            char c2 = substring.charAt(index2++);
            if (c1 == c2) {
                continue;
            }
            if (!ignoreCase) {
                return false;
            }
            if (Character.toUpperCase(c1) != Character.toUpperCase(c2)
                    && Character.toLowerCase(c1) != Character.toLowerCase(c2)) {
                return false;
            }
        }
        return true;
    }
}
\end{lstlisting}

==> listings/codec_CharSeq_ori_ori.tex <==
\textbf{}\begin{lstlisting}[style=Java, float, floatplacement=H, caption={Excerpt of \texttt{org.\allowbreak{}apache.\allowbreak{}commons.\allowbreak{}codec.\allowbreak{}binary.\allowbreak{}CharSequenceUtils}}, label={lst:charseq-ori}, escapechar=\¤,belowskip=-6\baselineskip]
public class CharSequenceUtils {
    static boolean regionMatches(final CharSequence cs, final boolean ignoreCase, final int thisStart,
            final CharSequence substring, final int start, final int length) {
        if (...) {
            [...]
        }
        int index1 = thisStart;
        int index2 = start;
        int tmpLen = length;
        while (tmpLen-- > 0) {
            char c1 = cs.charAt(index1++);
            char c2 = substring.charAt(index2++);
            if (c1 == c2) {
                continue;
            }
            if (!ignoreCase) {
                return false;
            }
            // The same check as in String.regionMatches():
            if (Character.toUpperCase(c1) != Character.toUpperCase(c2)
                    && Character.toLowerCase(c1) != Character.toLowerCase(c2)) {
                return false;
            }
        }
        return true;
    }
}
\end{lstlisting}

==> tables/CC-nonobf.tex <==
\begin{table}[htbp]
\caption{Cognitive Complexity of the original source code and code generated by decompilers.}
\scriptsize
\centering
    \begin{tabular}{lcccc}
		\hline
		\textsc{\textbf{Project name}} & \textsc{\textbf{Original}} & \textsc{\textbf{CFR}} & \textsc{\textbf{Fernflower}} & \textsc{\textbf{Jadx}}\\% & Commit ID\\
		\hline
        Bukkit	& $3527$ & $3313$ & $4724$ & $3645$\\% & f210234e59275330f83b994e199c76f6abd41ee7 \\
        Commons-codec & $1399$ & $1209$ & $1860$ & $1376$\\% & fe6dbee7524a5aa4160751155be2e8c975f66c68 \\
        Commons-collections	& $3711$ & $3471$ & $4995$ & $3399$\\% & a3503a1b569977dc6f8f136dcdcdabe49b8249c1 \\
        Commons-imaging	& $5066$ & $4741$ & $6921$ & $4726$\\% & 92440e4206a12ffd455def326c181058b53b6681 \\
        Commons-lang & $6281$ & $5965$ & $9132$ & $6435$\\% & 3482322192307199d4db1c66e921b7beb6e6dcb6 \\
        DiskLruCache & $171$ & $167$ & $248$ & $175$\\% & c2965c04a03d016c58323c41223d8e2808adf732 \\
        JavaPoet	& $135$ & $140$ & $153$ & $140$\\% & d39761f9ec25ca5bf3b7bf15d34fa2b831fed9c1 \\
        Joda time	& $4368$ & $4026$ & $5818$ & $4193$\\% & 8ddb3fb57078d57cfea00b1f588c9ffa8ffbec03 \\
        Jsoup	& $1351$ & $1226$ & $1553$ & $1362$\\% & ab7feede4eedee351f320896114394235c2395ef \\
        JUnit4	& $1241$ & $1141$ & $1455$ & $1228$\\% & 077f5c502a2494c3625941724ddcd5412a99ccc8 \\
        Mimecraft	& $33$ & $33$ & $39$ & $41$\\% & e7b3f9a764fc34cd473e6e2072cb5a995bec0bb2 \\
        Scribe Java	& $101$ & $86$ & $100$ & $87$\\% & e47e494ce39f9b180352fc9b5fd73c8b3ccce7f8 \\
        Spark & $277$ & $244$ & $314$ & $275$\\% & a19594a0e9d824c61996897cf8d1efcd9da43313 \\
        DcTest & $18$ & $17$ & $33$ & $37$\\
        \hline
        \textsc{\textbf{Total}} &  \textbf{$27679$} & \textbf{$25779$}  & \textbf{$37345$} & \textbf{$27115$}\\
        \hline
	\end{tabular}
	\label{tab:dataset}
    % \vspace{-0.5cm}
\end{table}

==> tables/CC_improved_overview.tex <==
\begin{table}[htbp]
\caption{Decompiled Cognitive Complexity of the original code and decompiled code.}
\scriptsize
\centering
    \setlength{\tabcolsep}{0.35em}
\resizebox{0.48\textwidth}{!}{
    \begin{tabular}{lccccc}
		\hline
		\textsc{\textbf{Project}} & \textsc{\textbf{\#File}} & \textsc{\textbf{Original}} & \textsc{\textbf{CFR}} & \textsc{\textbf{Fernflower}} & \textsc{\textbf{Jadx}}\\
		\hline
        Bukkit	            & $100$& $1277$& $1424$& $1488$& $1319$\\
        Commons-codec       & $26$ & $444$ & $631$ & $736$ & $545$ \\
        Commons-collections	& $32$ & $87$  & $110$ & $124$ & $101$ \\
        Commons-imaging	    & $86$ & $1039$& $1988$& $1989$& $1214$\\
        Commons-lang        & $28$ & $368$ & $596$ & $611$ & $523$ \\
        Joda time	        & $71$ & $942$ & $1356$& $1363$& $1146$\\
        Jsoup	            & $11$ & $602$ & $350$ & $334$ & $302$ \\
        Junit4	            & $36$ & $251$ & $305$ & $312$ & $279$ \\
        Mimecraft	        & $2$  & $25$  & $25$  & $29$  & $30$\\
        Scribe Java	        & $25$ & $126$ & $112$ & $100$ & $101$\\
        Spark               & $9$  & $42$ & $50$ & $45$ & $41$\\
        DcTest              & $3$  & $40$ & $27$ & $43$ & $32$\\
        \hline
        \textsc{\textbf{Total}} &  \textbf{$429$} &  \textbf{$5243$} & \textbf{$6974$}  & \textbf{$7174$} & \textbf{$5633$}\\
        \hline
	\end{tabular}
	\label{tab:dataset_CC_improved}
}
    % \vspace{-0.5cm}
\end{table}

==> tables/CC_overview.tex <==
\begin{table}[htbp]
\caption{Cognitive Complexity of the original code and decompiled code.}
\centering
    \setlength{\tabcolsep}{0.35em}
\resizebox{0.48\textwidth}{!}{
    \begin{tabular}{lccccc}
		\hline
		\textsc{\textbf{Project}} & \textsc{\textbf{\#File}} & \textsc{\textbf{Original}} & \textsc{\textbf{CFR}} & \textsc{\textbf{Fernflower}} & \textsc{\textbf{Jadx}}\\
		\hline
        Bukkit	& $100$ & $880$ & $837$ & $1158$ & $958$\\
        Commons-codec & $26$ & $373$ & $339$ & $574$ & $385$\\
        Commons-collections	& $32$ & $87$ & $86$ & $106$ & $85$\\
        Commons-imaging	& $86$ & $676$ & $642$ & $822$ & $676$\\
        Commons-lang & $28$ & $348$ & $348$ & $480$ & $385$\\
        Joda time	& $71$ & $815$ & $769$ & $1049$ & $782$\\
        Jsoup	& $11$ & $251$ & $214$ & $294$ & $226$\\
        Junit4	& $36$ & $234$ & $228$ & $260$ & $230$\\
        Mimecraft	& $2$ & $21$ & $21$ & $25$ & $30$\\
        Scribe Java	& $25$ & $75$ & $62$ & $72$ & $63$\\
        Spark & $9$ & $40$ & $38$ & $43$ & $39$\\
        DcTest & $3$ & $14$ & $13$ & $29$ & $30$\\
        \hline
        \textsc{\textbf{Total}} &  \textbf{$429$} &  \textbf{$3814$} & \textbf{$3597$}  & \textbf{$4912$} & \textbf{$3889$}\\
        \hline
	\end{tabular}
	\label{tab:dataset_CC}
}
    % \vspace{-0.5cm}
\end{table}

==> tables/acm_confusion_matrix_CC_improved_per_decompiler.tex <==
\begin{table*}[htbp]
    \caption{Confusion Matrix and metrics of the relative understandability indicated by the improved metric by decompilers} \label{tab:conf_matrix_CC_impr_per_decompiler}
  \begin{subtable}{0.28\linewidth}
    \caption{CFR} \label{tab:conf_matrix_CC_impr_cfr}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{c|c|c|c|c|}
            \multicolumn{2}{c}{} & \multicolumn{3}{c}{Actual} \\
            \cline{2-5}
             &  & Less & Equi & More \\
            \cline{2-5}
            \multirow{3}{*}{Pred} & Less & 94 & 17 & 0 \\
            \cline{2-5}
            & Equi & 16 & 259 & 4 \\
            \cline{2-5}
            & More & 0 & 9 & 30 \\
            \cline{2-5}
        \end{tabular}
    }
    % \caption{Table 1}
  \end{subtable}
  \hfill
  \begin{subtable}{0.28\linewidth}
    \caption{Fernflower} \label{tab:conf_matrix_CC_impr_fern}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{c|c|c|c|c|}
            \multicolumn{2}{c}{} & \multicolumn{3}{c}{Actual} \\
            \cline{2-5}
             &  & Less & Equi & More \\
            \cline{2-5}
            \multirow{3}{*}{Pred} & Less & 86 & 33 & 0 \\
            \cline{2-5}
            & Equi & 13 & 270 & 5 \\
            \cline{2-5}
            & More & 0 & 4 & 18 \\
            \cline{2-5}
        \end{tabular}
    }
    % \caption{Table 2}
  \end{subtable}
  \hfill
  \begin{subtable}{0.28\linewidth}
    \caption{Jadx} \label{tab:conf_matrix_CC_impr_jadx}
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{c|c|c|c|c|}
            \multicolumn{2}{c}{} & \multicolumn{3}{c}{Actual} \\
            \cline{2-5}
             &  & Less & Equi & More \\
            \cline{2-5}
            \multirow{3}{*}{Pred} & Less & 47 & 20 & 0 \\
            \cline{2-5}
            & Equi & 5 & 325 & 2 \\
            \cline{2-5}
            & More & 0 & 7 & 23 \\
            \cline{2-5}
        \end{tabular}
    }
    % \caption{Table 3}
  \end{subtable}
\end{table*}


==> tables/acm_confusion_matrix_CC_ori_per_decompiler.tex <==

\begin{table}
    \caption{Confusion Matrix of the relative understandability indicated by Cognitive Complexity for each decompiler}
  \begin{minipage}{0.3\textwidth} % 第一个 minipage，占 45% 的文本宽度
    \centering
    \begin{subtable}{\textwidth}
      \centering
        \caption{CFR}
        \begin{tabular}{c|c|c|c|c|}
            \multicolumn{2}{c}{} & \multicolumn{3}{c}{Actual} \\
            \cline{2-5}
             &  & Less & Equi & More \\
            \cline{2-5}
            \multirow{3}{*}{Pred} & Less & 4 & 0 & 0 \\
            \cline{2-5}
            & Equi & 97 & 289 & 22 \\
            \cline{2-5}
            & More & 8 & 5 & 4 \\
            \cline{2-5}
        \end{tabular}
        \label{tab:conf_matrix_CC_ori_cfr}
    \end{subtable}
  \end{minipage}
  \hfill % 空格分隔两个 minipage，使它们并排显示
  \begin{minipage}{0.3\textwidth} % 第二个 minipage，占 45% 的文本宽度
    \centering
    \begin{subtable}{\textwidth}
      \centering
        \caption{Fernflower}
        \begin{tabular}{c|c|c|c|c|}
            \multicolumn{2}{c}{} & \multicolumn{3}{c}{Actual} \\
            \cline{2-5}
             &  & Less & Equi & More \\
            \cline{2-5}
            \multirow{3}{*}{Pred} & Less & 47 & 23 & 3 \\
            \cline{2-5}
            & Equi & 52 & 288 & 15 \\
            \cline{2-5}
            & More & 0 & 0 & 1 \\
            \cline{2-5}
        \end{tabular}
        \label{tab:conf_matrix_CC_ori_fern}
    \end{subtable}
  \end{minipage}
  \hfill % 空格分隔两个 minipage，使它们并排显示
  \begin{minipage}{0.3\textwidth} % 第二个 minipage，占 45% 的文本宽度
    \centering
    \begin{subtable}{\textwidth}
      \centering
        \caption{Jadx}
        \begin{tabular}{c|c|c|c|c|}
            \multicolumn{2}{c}{} & \multicolumn{3}{c}{Actual} \\
            \cline{2-5}
             &  & Less & Equi & More \\
            \cline{2-5}
            \multirow{3}{*}{Pred} & Less & 15 & 9 & 1 \\
            \cline{2-5}
            & Equi & 33 & 337 & 21 \\
            \cline{2-5}
            & More & 4 & 3 & 6 \\
            \cline{2-5}
        \end{tabular}
        \label{tab:conf_matrix_CC_ori_jadx}
    \end{subtable}
  \end{minipage}
  \caption{Two Tables Side by Side}
\end{table}


==> tables/confusion_matrix_CC_CFR_ori.tex <==

\begin{table}[htbp]
    \caption{Confusion Matrix and metrics of the relative understandability of Cognitive Complexity of files generated by CFR}
    \centering
    \begin{subtable}[htbp]{1\linewidth}
        \centering
        \begin{tabular}{c|c|c|c|c|}
            \multicolumn{2}{c}{} & \multicolumn{3}{c}{Actual} \\
            \cline{2-5}
             &  & Less & Equivalent & More \\
            \cline{2-5}
            \multirow{3}{*}{Predicted} & Less & 61 & 176 & 9 \\
            \cline{2-5}
            & Equivalent & 32 & 842 & 11 \\
            \cline{2-5}
            & More & 4 & 34 & 10 \\
            \cline{2-5}
        \end{tabular}
        \caption{Confusion Matrix}
        \label{tab:conf_matrix_CC_cfr_ori}
    \end{subtable}
    \hfill

    \begin{subtable}[htbp]{1\linewidth}
        \centering
        \begin{tabular}{c|c|c|c|}
             & Less & Equivalent & More \\
            Precision & 0.2479 & 0.9514 & 0.2083 \\
            Recall & 0.6288 & 0.8003 & 0.3333 \\
            F1 & 0.3556 & 0.8693 & 0.2564 \\
            Balanced Accuracy &  0.7289 & 0.7308 & 0.6501 \\
        \end{tabular}
        \caption{Metrics}
        \label{tab:conf_matrix_CC_cfr_metric_ori}
    \end{subtable}
    
\end{table}


==> tables/confusion_matrix_CC_Fernflower_ori.tex <==

\begin{table}[htbp]
    \caption{Confusion Matrix and metrics of the relative understandability of Cognitive Complexity of files generated by Fernflower}
    \centering
    \begin{subtable}[htbp]{1\linewidth}
        \centering
        \begin{tabular}{c|c|c|c|c|}
            \multicolumn{2}{c}{} & \multicolumn{3}{c}{Actual} \\
            \cline{2-5}
             &  & Less & Equivalent & More \\
            \cline{2-5}
            \multirow{3}{*}{Predicted} & Less & 61 & 176 & 9 \\
            \cline{2-5}
            & Equivalent & 32 & 842 & 11 \\
            \cline{2-5}
            & More & 4 & 34 & 10 \\
            \cline{2-5}
        \end{tabular}
        \caption{Confusion Matrix}
        \label{tab:conf_matrix_CC_fern_ori}
    \end{subtable}
    \hfill

    \begin{subtable}[htbp]{1\linewidth}
        \centering
        \begin{tabular}{c|c|c|c|}
             & Less & Equivalent & More \\
            Precision & 0.2479 & 0.9514 & 0.2083 \\
            Recall & 0.6288 & 0.8003 & 0.3333 \\
            F1 & 0.3556 & 0.8693 & 0.2564 \\
            Balanced Accuracy &  0.7289 & 0.7308 & 0.6501 \\
        \end{tabular}
        \caption{Metrics}
        \label{tab:conf_matrix_CC_fern_metric_ori}
    \end{subtable}
    
\end{table}


==> tables/confusion_matrix_CC_Jadx_ori.tex <==

\begin{table}[htbp]
    \caption{Confusion Matrix and metrics of the relative understandability of Cognitive Complexity of files generated by Jadx}
    \centering
    \begin{subtable}[htbp]{1\linewidth}
        \centering
        \begin{tabular}{c|c|c|c|c|}
            \multicolumn{2}{c}{} & \multicolumn{3}{c}{Actual} \\
            \cline{2-5}
             &  & Less & Equivalent & More \\
            \cline{2-5}
            \multirow{3}{*}{Predicted} & Less & 61 & 176 & 9 \\
            \cline{2-5}
            & Equivalent & 32 & 842 & 11 \\
            \cline{2-5}
            & More & 4 & 34 & 10 \\
            \cline{2-5}
        \end{tabular}
        \caption{Confusion Matrix}
        \label{tab:conf_matrix_CC_jadx_ori}
    \end{subtable}
    \hfill

    \begin{subtable}[htbp]{1\linewidth}
        \centering
        \begin{tabular}{c|c|c|c|}
             & Less & Equivalent & More \\
            Precision & 0.2479 & 0.9514 & 0.2083 \\
            Recall & 0.6288 & 0.8003 & 0.3333 \\
            F1 & 0.3556 & 0.8693 & 0.2564 \\
            Balanced Accuracy &  0.7289 & 0.7308 & 0.6501 \\
        \end{tabular}
        \caption{Metrics}
        \label{tab:conf_matrix_CC_jadx_metric_ori}
    \end{subtable}
    
\end{table}


==> tables/confusion_matrix_CC_improved.tex <==

\begin{table}[htbp] \footnotesize
    \caption{Confusion Matrix and metrics of the relative understandability indicated by Cognitive Complexity\textsuperscript{D}.} 
    \label{tab:conf_matrix_CC_improved_all}
    \centering
    \begin{subtable}[htbp]{0.47\linewidth}
        \centering
        \caption{Confusion Matrix}
        \setlength{\tabcolsep}{0.45em}
            \begin{tabular}{c|c|c|c|c|}
                \multicolumn{2}{c}{} & \multicolumn{3}{c}{Actual} \\
                \cline{2-5}
                 &  & Less & Equi & More \\
                \cline{2-5}
                \multirow{3}{*}{Pred} & Less & 227 & 70 & 0 \\
                \cline{2-5}
                & Equi & 34 & 854 & 11 \\
                \cline{2-5}
                & More & 0 & 20 & 71 \\
                \cline{2-5}
            \end{tabular}
        \label{tab:conf_matrix_CC_improved}
    \end{subtable}
    \hfill
    \vspace{0.2cm}
    \begin{subtable}[htbp]{0.49\linewidth}  \footnotesize
    \centering
    \caption{Metrics}
    \setlength{\tabcolsep}{0.35em}
        \begin{tabular}{c ccc}
                    &       &       &       \\
        \hline
                    & Less  & Equi  & More  \\
        \hline
            Precision & 0.7643 & 0.9499 & 0.7802 \\
            Recall  & 0.8697 & 0.9046 & 0.8658 \\
            F1      & 0.8136 & 0.9267 & 0.8208 \\
        \hline
        \end{tabular}
    \label{tab:conf_matrix_CC_metric_improved}
    \end{subtable}
\vspace{-0.5cm}
\end{table}



==> tables/confusion_matrix_CC_improved_per_decompiler.tex <==
\begin{table*}[htbp]
    \caption{Confusion Matrix and metrics of the relative understandability indicated by the improved metric by decompilers.} \label{tab:conf_matrix_CC_impr_per_decompiler}
\centering
  \begin{subtable}{0.3\linewidth}  \footnotesize
    \caption{CFR} \label{tab:conf_matrix_CC_impr_cfr}
    \setlength{\tabcolsep}{0.45em}
        \begin{tabular}{c|c|c|c|c|}
            \multicolumn{2}{c}{} & \multicolumn{3}{c}{Actual} \\
            \cline{2-5}
             &  & Less & Equi & More \\
            \cline{2-5}
            \multirow{3}{*}{Pred} & Less & 94 & 17 & 0 \\
            \cline{2-5}
            & Equi & 16 & 259 & 4 \\
            \cline{2-5}
            & More & 0 & 9 & 30 \\
            \cline{2-5}
        \end{tabular}
    % \caption{Table 1}
  \end{subtable}
  % \hfill
  \begin{subtable}{0.3\linewidth}  \footnotesize
    \caption{Fernflower} \label{tab:conf_matrix_CC_impr_fern}
    \setlength{\tabcolsep}{0.45em}
        \begin{tabular}{c|c|c|c|c|}
            \multicolumn{2}{c}{} & \multicolumn{3}{c}{Actual} \\
            \cline{2-5}
             &  & Less & Equi & More \\
            \cline{2-5}
            \multirow{3}{*}{Pred} & Less & 86 & 33 & 0 \\
            \cline{2-5}
            & Equi & 13 & 270 & 5 \\
            \cline{2-5}
            & More & 0 & 4 & 18 \\
            \cline{2-5}
        \end{tabular}
    % \caption{Table 2}
  \end{subtable}
  % \hfill
  \begin{subtable}{0.3\linewidth}  \footnotesize
    \caption{Jadx} \label{tab:conf_matrix_CC_impr_jadx}
    \setlength{\tabcolsep}{0.45em}
        \begin{tabular}{c|c|c|c|c|}
            \multicolumn{2}{c}{} & \multicolumn{3}{c}{Actual} \\
            \cline{2-5}
             &  & Less & Equi & More \\
            \cline{2-5}
            \multirow{3}{*}{Pred} & Less & 47 & 20 & 0 \\
            \cline{2-5}
            & Equi & 5 & 325 & 2 \\
            \cline{2-5}
            & More & 0 & 7 & 23 \\
            \cline{2-5}
        \end{tabular}
    % \caption{Table 3}
  \end{subtable}
\end{table*}


==> tables/confusion_matrix_CC_ori.tex <==

\begin{table}[htbp]
    \caption{Confusion Matrix and metrics of the relative understandability of Cognitive Complexity of all files}
    \centering
    \begin{subtable}[htbp]{1\linewidth}
        \centering
        \caption{Confusion Matrix}
        \begin{tabular}{c|c|c|c|c|}
            \multicolumn{2}{c}{} & \multicolumn{3}{c}{Actual} \\
            \cline{2-5}
             &  & Less & Equivalent & More \\
            \cline{2-5}
            \multirow{3}{*}{Predicted} & Less & 66 & 32 & 4 \\
            \cline{2-5}
            & Equivalent & 182 & 905 & 67 \\
            \cline{2-5}
            & More & 12 & 8 & 11 \\
            \cline{2-5}
        \end{tabular}
        \label{tab:conf_matrix_CC_ori}
    \end{subtable}
    \hfill
    \vspace{0.2cm}
    \begin{subtable}[htbp]{1\linewidth}
        \centering
        \caption{Metrics}
        \begin{tabular}{c|ccc}
            \hline
             & Less & Equivalent & More \\ \hline
            Precision & 0.6470 & 0.7842 & 0.3548 \\
            Recall & 0.2538 & 0.9577 & 0.1341 \\
            F1 & 0.3646 & 0.8623 & 0.1947 \\
            % Balanced Accuracy &  0.6094 & 0.6148 & 0.5588 \\
            \hline
        \end{tabular}
        \label{tab:conf_matrix_CC_metric_ori}
    \end{subtable}
    
\end{table}


==> tables/confusion_matrix_CC_ori_per_decompiler.tex <==
\begin{table*}[tbp]
    \caption{Confusion Matrix of relative understandability indicated by Cognitive Complexity for each decompiler.} \label{tab:conf_matrix_CC_ori_per_decompiler} 
\centering
  \begin{subtable}{0.3\linewidth} \footnotesize
    \caption{CFR} \label{tab:conf_matrix_CC_ori_cfr}
    \setlength{\tabcolsep}{0.45em}
        \begin{tabular}{c|c|c|c|c|}
            \multicolumn{2}{c}{} & \multicolumn{3}{c}{Actual} \\
            \cline{2-5}
             &  & Less & Equi & More \\
            \cline{2-5}
            \multirow{3}{*}{Pred} & Less & 4 & 0 & 0 \\
            \cline{2-5}
            & Equi & 98 & 278 & 32 \\
            \cline{2-5}
            & More & 8 & 7 & 2 \\
            \cline{2-5}
        \end{tabular}
    % \caption{Table 1}
  \end{subtable}
  % \hfill
  \begin{subtable}{0.3\linewidth} \footnotesize
    \caption{Fernflower} \label{tab:conf_matrix_CC_ori_fern}
    \setlength{\tabcolsep}{0.45em}
        \begin{tabular}{c|c|c|c|c|}
            \multicolumn{2}{c}{} & \multicolumn{3}{c}{Actual} \\
            \cline{2-5}
             &  & Less & Equi & More \\
            \cline{2-5}
            \multirow{3}{*}{Pred} & Less & 48 & 22 & 3 \\
            \cline{2-5}
            & Equi & 51 & 284 & 20 \\
            \cline{2-5}
            & More & 0 & 1 & 0 \\
            \cline{2-5}
        \end{tabular}
    % \caption{Table 2}
  \end{subtable}
  % \hfill
  \begin{subtable}{0.3\linewidth} \footnotesize
    \caption{Jadx} \label{tab:conf_matrix_CC_ori_jadx}
    \setlength{\tabcolsep}{0.45em}
        \begin{tabular}{c|c|c|c|c|}
            \multicolumn{2}{c}{} & \multicolumn{3}{c}{Actual} \\
            \cline{2-5}
             &  & Less & Equi & More \\
            \cline{2-5}
            \multirow{3}{*}{Pred} & Less & 15 & 9 & 1 \\
            \cline{2-5}
            & Equi & 33 & 338 & 20 \\
            \cline{2-5}
            & More & 4 & 5 & 4 \\
            \cline{2-5}
        \end{tabular}
    % \caption{Table 3}
  \end{subtable}
\end{table*}

==> tables/confusion_matrix_ngram_ori.tex <==

\begin{table}[htbp]
    \caption{Confusion Matrix and metrics of the relative understandability of perplexity of all files}
    \centering
    \begin{subtable}[htbp]{1\linewidth}
        \centering
        \caption{Confusion Matrix}
        \begin{tabular}{c|c|c|c|c|}
            \multicolumn{2}{c}{} & \multicolumn{3}{c}{Actual} \\
            \cline{2-5}
             &  & Less & Equivalent & More \\
            \cline{2-5}
            \multirow{3}{*}{Predicted} & Less & 62 & 105 & 1 \\
            \cline{2-5}
            & Equivalent & 188 & 797 & 73 \\
            \cline{2-5}
            & More & 10 & 43 & 8 \\
            \cline{2-5}
        \end{tabular}
        \label{tab:conf_matrix_ngram_ori}
    \end{subtable}
    \hfill
    \vspace{0.2cm}
    \begin{subtable}[htbp]{1\linewidth}
    \centering
    \caption{Metrics}
    \begin{tabular}{c|ccc}
        \hline
         & Less & Equivalent & More \\
        \hline
        Precision & 0.3690 & 0.7533 & 0.1311 \\
        Recall & 0.2384 & 0.8433 & 0.0976 \\
        F1 & 0.2897 & 0.7958 & 0.1119 \\
        \hline
    \end{tabular}
    \label{tab:conf_matrix_ngram_metric_ori}
    \end{subtable}
% \vspace{-0.5cm}
\end{table}


==> tables/confusion_matrix_ngram_ori_per_decompiler.tex <==
\begin{table*}[tbp]
    \caption{Confusion Matrix of relative understandability indicated by perplexity for each decompiler.}
 \label{tab:conf_matrix_ngram_ori_per_decompiler}
\centering
  \begin{subtable}{0.3\linewidth} \footnotesize
    \caption{CFR} 
    \setlength{\tabcolsep}{0.45em}
    \label{tab:conf_matrix_ngram_ori_cfr}
        \begin{tabular}{c|c|c|c|c|}
            \multicolumn{2}{c}{} & \multicolumn{3}{c}{Actual} \\
            \cline{2-5}
             &  & Less & Equi & More \\
            \cline{2-5}
            \multirow{3}{*}{Pred} & Less & 32 & 41 & 0 \\
            \cline{2-5}
            & Equi & 74 & 228 & 30 \\
            \cline{2-5}
            & More & 4 & 16 & 4 \\
            \cline{2-5}
        \end{tabular}
    % \caption{Table 1}
  \end{subtable}
  % \hfill
  \begin{subtable}{0.3\linewidth} \footnotesize
    \caption{Fernflower} 
    \setlength{\tabcolsep}{0.45em}
    \label{tab:conf_matrix_ngram_ori_fern}
        \begin{tabular}{c|c|c|c|c|}
            \multicolumn{2}{c}{} & \multicolumn{3}{c}{Actual} \\
            \cline{2-5}
             &  & Less & Equi & More \\
            \cline{2-5}
            \multirow{3}{*}{Pred} & Less & 18 & 43 & 0 \\
            \cline{2-5}
            & Equi & 78 & 256 & 21 \\
            \cline{2-5}
            & More & 3 & 8 & 2 \\
            \cline{2-5}
        \end{tabular}
    % \caption{Table 2}
  \end{subtable}
  % \hfill
  \begin{subtable}{0.3\linewidth} \footnotesize
    \caption{Jadx}
    \setlength{\tabcolsep}{0.45em}
    \label{tab:conf_matrix_ngram_ori_jadx}
        \begin{tabular}{c|c|c|c|c|}
            \multicolumn{2}{c}{} & \multicolumn{3}{c}{Actual} \\
            \cline{2-5}
             &  & Less & Equi & More \\
            \cline{2-5}
            \multirow{3}{*}{Pred} & Less & 12 & 21 & 1 \\
            \cline{2-5}
            & Equi & 37 & 312 & 22 \\
            \cline{2-5}
            & More & 3 & 19 & 2 \\
            \cline{2-5}
        \end{tabular}
    % \caption{Table 3}
  \end{subtable} 
  \vspace{-0.2cm}
\end{table*}

==> tables/decompilers.tex <==
\begin{table}[htbp]
\caption{Characteristics of three decompilers.}
\scriptsize
    \setlength{\tabcolsep}{0.35em}
\centering
    \begin{tabular}{lcccc}
		\hline
		\textsc{\textbf{Decompiler}} & \textsc{\textbf{Version}} & \textsc{\textbf{ \#commits}} & \textsc{\textbf{\#stars}} & \textsc{\textbf{\#LOC}}\\
		\hline
            CFR	& 0.152 & 1878 & 1.7K & 66173\\
            Fernflower & - & 637 & 3K & 57264\\
            Jadx	& 1.4.5 & 1861 & 36K & 69214\\
		\hline
	\end{tabular}
	\label{tab:decompilers}
    % \vspace{-0.5cm}
\end{table}

==> tables/perplexity-filter.tex <==
\begin{table}[htbp]
\caption{Perplexity of the original code and decompiled code.}
\scriptsize
\centering
\resizebox{0.48\textwidth}{!}{
    \begin{tabular}{lccccc}
	\hline
	\textsc{\textbf{Project name}} & \textsc{\textbf{\#File}} & \textsc{\textbf{Original}} & \textsc{\textbf{CFR}} & \textsc{\textbf{Fernflower}} & \textsc{\textbf{Jadx}}\\
	\hline
        Bukkit	& $100$ & $14241.1$ & $14222.1$ & $13610.5$ & $13536.3$\\
        Commons-codec & $26$ & $1189.1$ & $1244.6$ & $1197.4$ & $1392.9$\\
        Commons-collections	& $32$ & $1158.9$ & $1131.2$ & $1311.5$ & $1113.0$\\
        Commons-imaging	& $86$ & $11834.7$ & $13205.3$ & $12496.0$ & $13216.5$\\
        Commons-lang & $28$ & $1242.6$ & $1481.3$ & $1632.4$ & $1338.1$\\
        Joda time	& $71$ & $10447.6$ & $8817.9$ & $9248.5$ & $8589.4$\\
        Jsoup	& $11$ & $978.7$ & $917.6$ & $876.4$ & $833.2$\\
        Junit4	& $36$ & $1567.0$ & $1379.1$ & $1586.6$ & $1436.8$\\
        Mimecraft	& $2$ & $57.2$ & $49.0$ & $53.0$ & $48.5$\\
        Scribe Java	& $25$ & $2622.3$ & $3557.7$ & $3740.4$ & $3099.7$\\
        Spark & $9$ & $265.7$ & $353.4$ & $281.8$ & $268.3$\\
        DcTest & $3$ & $59.4$ & $68.0$ & $98.1$ & $72.9$\\
        \hline
        \textsc{\textbf{Total}} &  \textbf{$429$} &  \textbf{$45664.9$} & \textbf{$46382.4$}  & \textbf{$46049.2$} & \textbf{$44949.3$}\\
        \hline
    \end{tabular} \label{tab:dataset_perplexity}
}
% \vspace{-0.5cm}
\end{table}

==> tables/understandability_annotated.tex <==
\begin{table}[htbp]
\caption{Understandability of the decompiled files generated by different decompilers compared to the corresponding original files.}
\scriptsize
\centering
\resizebox{0.48\textwidth}{!}{
    \begin{tabular}{l|cccc}
		\hline
		 & \textsc{\textbf{CFR}} & \textsc{\textbf{Fernflower}} & \textsc{\textbf{Jadx}} & \textsc{\textbf{All}} \\ \hline
        \#Less 	        & $109(25\%)$   & $99(23\%)$  & $52(12\%)$ & $260(20\%)$ \\
        \#Equivalent    & $285(66\%) $  & $311(72\%)$ & $349(81\%)$& $945(73\%)$ \\
        \#More 	        & $35(8\%) $    & $19(4\%)$   & $28(7\%)$  & $82(6\%)$   \\ \hline
\textsc{\textbf{Total}} & $429(100\%) $ & $429(100\%)$&$429(100\%)$& $1287(100\%)$ \\
        \hline
	\end{tabular}
	\label{tab:dataset_annotated}
}
% \vspace{-0.5cm}
\end{table}
